OLIVES Dataset: Ophthalmic Labels for Investigating Visual Eye Semantics

Clinical diagnosis of the eye is performed over multifarious data modalities including scalar clinical labels, vectorized biomarkers, two-dimensional fundus images, and three-dimensional Optical Coherence Tomography (OCT) scans. Clinical practitioners use all available data modalities for diagnosing and treating eye diseases like Diabetic Retinopathy (DR) or Diabetic Macular Edema (DME). Enabling usage of machine learning algorithms within the ophthalmic medical domain requires research into the relationships and interactions between all relevant data over a treatment period. Existing datasets are limited in that they neither provide data nor consider the explicit relationship modeling between the data modalities. In this paper, we introduce the Ophthalmic Labels for Investigating Visual Eye Semantics (OLIVES) dataset that addresses the above limitation. This is the first OCT and near-IR fundus dataset that includes clinical labels, biomarker labels, disease labels, and time-series patient treatment information from associated clinical trials. The dataset consists of 1268 near-IR fundus images each with at least 49 OCT scans, and 16 biomarkers, along with 4 clinical labels and a disease diagnosis of DR or DME. In total, there are 96 eyes' data averaged over a period of at least two years with each eye treated for an average of 66 weeks and 7 injections. We benchmark the utility of OLIVES dataset for ophthalmic data as well as provide benchmarks and concrete research directions for core and emerging machine learning paradigms within medical image analysis.

==> Sections/Extras.tex <==
\paragraph{Ethical Considerations}
\textcolor{blue}{ Within any medical research, ethical concerns exist surrounding the usage of data. The authors of \cite{chen2021ethical} identify that many ethical concerns are tied to the potential of machine learning to amplify existing inequalities within healthcare itself. This work contextualizes this issue into five potential areas where this could occur: problem selection, data collection, outcome definition, algorithm development, and post-deployment considerations. Within the context of our work an awareness that the data may not extend to all subsets of the population is necessary for ethical development of machine learning algorithms. For example, the data was collected as part of clinical trials at the retinal consultants of Texas, which implies the participants had the time and means to be part of these trials, which may not always be the case for disadvantaged groups. Additionally, it can readily be assumed that data collected at a renowned facility, such as this, may be of a higher quality than that found at institutions without access to state of the art imaging technologies. The potential problem with this is that the benefit that machine learning could provide will be restricted to small subsets of society unless thought is put into preventing this disparity. We believe that while this dataset is important to the advancement of healthcare research, an understanding of inequality in health is needed to prevent further exacerbation of this issue when utilizing this dataset.  
}
